Optimizing Server Locations in Spatial Queues: Parametric and Nonparametric Bayesian Optimization

This paper presents a new model for solving the optimal server location problem in a spatial hypercube queueing model. Unlike deterministic location models, our approach accounts for server availability, varying utilization levels, and dependencies across servers. We prove that the problem is NP-hard and establish lower and upper bounds, as well as asymptotic results, by relating it to special cases of the classical $p$-Median problem. To address the computational challenge, we propose two Bayesian optimization approaches: (i) a parametric approach based on a sparse Bayesian linear model with second-order interactions, and (ii) a nonparametric approach using a Gaussian process surrogate with the $p$-Median objective as the prior mean function. We prove that both methods achieve sublinear regret and converge to the optimal solution. Numerical experiments and a case study using real-world data from the St. Paul, Minnesota, emergency response system show that our approaches consistently identify optimal solutions and outperform all baseline methods.

==> 92-st_further.tex <==

\section{Further Examination of the St. Paul Case Study Results}

\cmt{We may remove this.}

\subsection{Experiment Setup}\label{ssec: exp_setup}
For GP-based methods, we initialize with edge length $d_0=20$ and set hyperparameters as follows: $n_s=3$, $n_f=10$, $\alpha_s=1.5$, $\alpha_f=2/3$, and $\beta = 25$. All experiments were conducted on an Apple M1 system with 16GB RAM, with consistent hyperparameters across both simulation experiments and the case study in Section~\ref{sec_realdata}.


\subsection{An Alternative Objective Function: Fraction of Responses over a Time Threshold}
\label{ssec:alternative_objective}

Beyond average response time, a critical EMS performance metric is the fraction of calls exceeding a response time threshold~\citep{blackwell2002response,ingolfsson2008optimal,nasrollahzadeh2018real}. We therefore reformulate our optimization problem to minimize this fraction:
\begin{equation}
   \min_{\boldsymbol{x}} \sum_{i \in I} \sum_{j \in J}\mathbbm{1}\{\tau_i + t_{i j}\geq \bar{T}\} q_{i j}(\boldsymbol{x}),
\end{equation}
where $\bar{T}$ represents the response time threshold, and $q_{ij}(\boldsymbol{x})$ is the service allocation probability from \eqref{eq_qij}.

Our approach demonstrates significant advantages over traditional methods, as shown in Figure~\ref{fig_3_lambda}. At an 8-minute threshold, GP-$p$M and SparBL achieve a 7.83\% late-response rate compared to the $p$-Median's 10.8\% (38.5\% higher). This performance gap widens to 50\% at a 9-minute threshold (3.88\% vs. 5.76\%).


\begin{figure}[hbtp]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Map/late_call_7.png}
        \caption{7-minute response time threshold objective.}
    \label{fig_threshold}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Map/late_call_8.png}
        \caption{8-minute response time threshold objective.}
        \label{fig_8min}
    \end{subfigure}
    \caption{Location Results for Alternative Objective Function}
\end{figure}


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/output.jpg}
        \caption{Percentage (\%) of calls exceeding time thresholds.}
    \label{fig_3_lambda}
\end{figure}

Figure~\ref{fig_threshold} demonstrates the spatial configuration generated by our method when optimizing for a 7-minute response time threshold, contrasting sharply with the average-time-optimal layout in Figure~\ref{fig_StPaul_0}. The threshold-based solution exhibits two strategic relocations: (i) the tract 59-60 border unit shifts outward to tract 62, and (ii) the central tract 38-67 hub unit disperses northeastward to tract 24. These movements reflect a systematic rebalancing from demand-centric clustering to coverage-oriented dispersion. While average-time minimization aggregates units near high-call-density zones, threshold optimization induces more geographically equitable distributions to mitigate long-tail response delays.

Figure \ref{fig_8min} displays the unit locations when the time threshold is set to 8 minutes. We compare this figure to Figure \ref{fig_compare_cur_config} in the main text, which represents the optimal unit locations based on average response time.


In this configuration, one unit moves compared to the optimal arrangement. Specifically, the unit previously located at the junction of tracts 59 and 60 moves to tract 66 in the lower left area. This shift enables the unit at tract 68 to serve tracts 59, 60, 61, and nearby regions within the 8-minute response time. The relocated unit at tract 66 now satisfies the 8-minute threshold requirement for tracts in the lower left region of the city.

Compared to Figure~\ref{fig_threshold}, where the time threshold is 7 minutes, there is a notable change with the unit at the intersection of tracts 53, 62, and 63 moved back to the city center. This adjustment was made because these tracts, along with other adjacent ones, are now within an 8-minute travel distance from the unit in the city center. As a result, the revised time threshold of 8 minutes is now satisfied without the need for a dedicated unit in that region. %This example shows how our approach can handle different time threshold requirements taking into account the distribution of emergency calls and potential ambulance locations.

==> Tables/bounds.tex <==
% \begin{table}[!h]
% 	\centering
%         \caption{Numerical results of lower and upper bounds for different service rates}
% 	\renewcommand{\arraystretch}{0.7}
% 		\begin{tabular}{c| c |c |c |c} 
% 			 \hline $\mu$ & Optimum (min) & Our Approach (min) & Lower Bound (min) & Upper Bound  (min)\\
% 			\hline 
% 			{10}&{8.247}&{8.247}&{5.326}&{8.879}\\

% 			{15}&{7.389}&{7.389}&{5.326}&{7.737}\\

% 			{20}&{6.825}&{6.825}&{5.326}&{6.984}\\

% 			{25}&{6.425}&{6.425}&{5.326}&{6.532}\\

% 			{30}&{6.170}&{6.170}&{5.326}&{6.256}\\

% 			{$42^*$}&{5.863}&{5.863}&{5.326}&{5.916}\\
% 			{50}&{5.763}&{5.763}&{5.326}&{5.803}\\
%    			{100}&{5.538}&{5.538}&{5.326}&{5.543}\\
%       		{150}&{5.467}&{5.467}&{5.326}&{5.467}\\
%          	{200}&{5.430}&{5.430}&{5.326}&{5.430}\\
% 			{300}&{5.395}&{5.395}&{5.326}&{5.395}\\
% 			{500}&{5.367}&{5.367}&{5.326}&{5.367}\\
% 			{1000}&{5.346}&{5.346}&{5.326}&{5.346}\\
% 			\hline
% 		\end{tabular}
% 		\label{tab_bound}
% \end{table}


\begin{table}[!ht]
\caption{Numerical results of lower and upper bounds for different service rates. Number with asterisk represent the original service rate.}
\centering
\footnotesize
        {\def\arraystretch{1}  %change the number for increasing or decreasing the spacing.
            %\scriptsize %uncomment this for changing the font size
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}cccccc}
\hline
\hline
$\mu$ & Opt (min) & GP-$p$M & SparBL & Lower Bound (min) & Upper Bound (min) \\
\hline 
{10}      & {8.25} & {8.25} & {8.25} & {5.33} & {8.88} \\
{15}      & {7.39} & {7.39} & {7.39} & {5.33} & {7.74} \\
{20}      & {6.83} & {6.83} & {6.83} & {5.33} & {6.98} \\
{25}      & {6.43} & {6.43} & {6.43} & {5.33} & {6.53} \\
{30}      & {6.17} & {6.17} & {6.17} & {5.33} & {6.26} \\
{$42^*$}  & {5.86} & {5.86} & {5.86} & {5.33} & {5.92} \\
{50}      & {5.76} & {5.76} & {5.76} & {5.33} & {5.80} \\
{100}     & {5.54} & {5.54} & {5.54} & {5.33} & {5.54} \\
{150}     & {5.47} & {5.47} & {5.47} & {5.33} & {5.47} \\
{200}     & {5.43} & {5.43} & {5.43} & {5.33} & {5.43} \\
{300}     & {5.40} & {5.40} & {5.40} & {5.33} & {5.40} \\
{500}     & {5.37} & {5.37} & {5.37} & {5.33} & {5.37} \\
{1000}    & {5.35} & {5.35} & {5.35} & {5.33} & {5.35} \\
\hline
\hline
\end{tabular*}
\label{tab_bound}
}
\end{table}

% \begin{table}[!h]
% 	\centering
%         \footnotesize
%         \caption{Numerical results of lower and upper bounds for different service rates}
% 	\renewcommand{\arraystretch}{1}
% 		\begin{tabular}{ccccc} 
% 			 \hline $\mu$ & Optimum (min) & Our Approach (min) & Lower Bound (min) & Upper Bound  (min)\\
% 			\hline 
% 			{10}&{8.25}&{8.25}&{5.33}&{8.88}\\

% 			{15}&{7.39}&{7.39}&{5.33}&{7.74}\\

% 			{20}&{6.83}&{6.83}&{5.33}&{6.98}\\

% 			{25}&{6.43}&{6.43}&{5.33}&{6.53}\\

% 			{30}&{6.17}&{6.17}&{5.33}&{6.26}\\

% 			{$42^*$}&{5.86}&{5.86}&{5.33}&{5.92}\\
% 			{50}&{5.76}&{5.76}&{5.33}&{5.80}\\
%    			{100}&{5.54}&{5.54}&{5.33}&{5.54}\\
%       		{150}&{5.47}&{5.47}&{5.33}&{5.47}\\
%          	{200}&{5.43}&{5.43}&{5.33}&{5.43}\\
% 			{300}&{5.40}&{5.40}&{5.33}&{5.40}\\
% 			{500}&{5.37}&{5.37}&{5.33}&{5.37}\\
% 			{1000}&{5.35}&{5.35}&{5.33}&{5.35}\\
% 			\hline
% 		\end{tabular}
% 		\label{tab_bound}
% \end{table}

==> Tables/params.tex <==
\begin{table}[!h]
	\centering
	\renewcommand{\arraystretch}{0.7}
		\begin{tabular}{||c| c |c | c| c |c |c | c |c||} 
			\hline $l_1$
			& $l_2$ & $l_3$ & $l_4$ & $l_5$ & $l_6$ & $l_7$ & $l_8$ & $l_9$ \\
			\hline
			{0.1508}&{0.4488}&{0.4503}&0.0117&0.0114& 0.4346 &0.0138&0.1631&0.4352\\
			
			\hline\hline
			$l_{10}$&$l_{11}$ & $l_{12}$& $l_{13}$&$l_{14}$&$l_{15}$&$l_{16}$&$l_{17}$&$\gamma$\\
			\hline
			
			0.0117&0.0126& 0.3277&0.0117&0.0113&0.0116&0.0117&0.0111 & 0.4879\\
			
			\hline
		\end{tabular}
		\caption{Parameter values in the kernel}
		
		\vspace{-0.6cm}
		
\end{table}

==> Tables/peak_hours.tex <==
\begin{table}[!h]
	\centering
        \caption{Results of adding additional units during peak hours}
	\renewcommand{\arraystretch}{0.7}
		\begin{tabular}{c| c |c } 
			 \hline \# EMS Units & Our Approach (min) & p-Median (min) \\
			\hline 
			{10 (+1 unit)}&{6.35}&{6.59}\\

			{11 (+2 units)}&{6.10}&{6.19}\\

			{12 (+3 units)}&{5.87}&{5.92}\\

			\hline
		\end{tabular}
		\label{tab_peak}
\end{table}

==> Tables/peak_hours_1.4_lambda.tex <==
\begin{table}[!h]
	\centering
        \caption{Results of adding additional units during peak hours}
	\renewcommand{\arraystretch}{0.7}
		\begin{tabular}{c | c |c } 
			 \hline \# EMS Units & Our Approach (min) & p-Median (min) \\
			\hline 
                {9 (original)}&{6.16}&{6.25}\\
			{10 (+1 unit)}&{5.93}&{6.03}\\

			{11 (+2 units)}&{5.74}&{5.75}\\

			{12 (+3 units)}&{5.56}&{5.57}\\

			\hline
		\end{tabular}
		\label{tab_peak}
\end{table}

==> algorithms/BOFTR.tex <==
\begin{algorithm}
\caption{Bayesian Optimization Solution}
\label{BO_algo}
{\fontsize{10}{16}\selectfont
\begin{algorithmic}[1]
\setstretch{0}
\State \textbf{Input:} Initial sample size $\mathcal{T}$; initial edge-length $d_0$; evaluation budget $T$; $\alpha_s, \alpha_f, n_s, n_f$. 
\State Randomly select $\mathcal{T}$ initial samples $\boldsymbol{X}_{\mathcal{T}} = \{\boldsymbol{x}_1, ..., \boldsymbol{x}_{\mathcal{T}}\}$ and evaluate $\boldsymbol{Y}_{\mathcal{T}} = \{f(\boldsymbol{x}_1),f(\boldsymbol{x}_2),\cdots, f(\boldsymbol{x}_{\mathcal{T}})\}$
\State Initialize the current best solution: $y^* \leftarrow \min f(\boldsymbol{x}_i)$, $\boldsymbol{x^*} \leftarrow \arg \min f(\boldsymbol{x}_i)$, $t \leftarrow \mathcal{T}+1$, restart $\leftarrow True$.
\While {$t < T$}
\If{restart is True}
\State Reset edge-length $d \leftarrow d_0$, and set restart $\leftarrow$ False.
% \If{$k = 0$}
% \State Initialize observed data $\boldsymbol{X}_t \leftarrow \boldsymbol{X}_I$, $\boldsymbol{Y}_t \leftarrow  \{f(\boldsymbol{x})\ |\ \boldsymbol{x}\in \boldsymbol{X}_I\}$.
% \EndIf
\State Update the surrogate Gaussian process model with the latest observations $(\boldsymbol{X}_{t-1}, \boldsymbol{Y}_{t-1})$.
\State Determine a new center of the feasible trust region $\boldsymbol{x^c}$ using (\ref{eq_center}).
\Else

%\State Select next candidate $\boldsymbol{x_t}$ within $TR_t$ by the surrogate model $\boldsymbol{x_t} = \underset{\boldsymbol{x}\in TR(\boldsymbol{x^*_t})}{\mathrm{argmin}} \hat{f}(\boldsymbol{x})$.

\State Perform \textit{Adaptive Swapping} in the feasible trust region to obtain the next candidate solution $\boldsymbol{x_t}$.

\State Evaluate the objective function $f(\boldsymbol{x_t})$ and store the outcome $y_t=f(\boldsymbol{x_t})$.

\State Update $\boldsymbol{X}_t \leftarrow \boldsymbol{X}_{t-1}\cup \{\boldsymbol{x_t}\}$, $\boldsymbol{Y}_t \leftarrow \boldsymbol{Y}_{t-1}\cup \{y_t\}$, and the surrogate Gaussian process model.

\If{$y_t < y^*$} 
\State Update the best known solution: $y^* \leftarrow y_t, \boldsymbol{x^*} \leftarrow \boldsymbol{x}_t$
\EndIf

\If{$y^*$ has improved $n_s$ times} 
\State Increase the edge-length $d \leftarrow d \alpha_s$
\EndIf

\If{$y^*$ remains unchanged for $n_f$ consecutive iterations}
\State Reduce the edge-length $d \leftarrow d \alpha_f$
\EndIf

\EndIf
\If{$\lfloor d \rfloor < 2$}
\State Set restart $\leftarrow$ True.
\EndIf
\State Move to the next iteration $t \leftarrow t + 1$.
\EndWhile
\Statex \textbf{Output:}  Best solution found $\boldsymbol{x^*}$ and its corresponding objective function value $y^*$.
\end{algorithmic}}
\end{algorithm}

==> exps/99-algo.tex <==

\section{Algorithms}

\begin{algorithm}[H]
\DontPrintSemicolon
  
  \KwInput{Your Input}
  \KwOutput{Your output}
  \KwData{Testing set $x$}
  $\sum_{i=1}^{\infty} := 0$ \tcp*{this is a comment}
  \tcc{Now this is an if...else conditional loop}
  \If{Condition 1}
    {
        Do something    \tcp*{this is another comment}
        \If{sub-Condition}
        {Do a lot}
    }
    \ElseIf{Condition 2}
    {
    	Do Otherwise \;
        \tcc{Now this is a for loop}
        \For{sequence}    
        { 
        	loop instructions
        }
    }
    \Else
    {
    	Do the rest
    }
    
    \tcc{Now this is a While loop}
   \While{Condition}
   {
   		Do something\;
   }

\caption{Example code}
\end{algorithm}

==> exps/99-codes.tex <==
%%
%%  Spinning Up
%%

% \lstinputlisting[language=Octave]{BitXorMatrix.m}

\section{AWS Setup}

To set up AWS, follow the \href{https://course.fast.ai/start_aws.html}{tutorial} by FastAI. Once an instance is created and started, use the following codes to start virtual environment and launch Jupyter notebook. 

\begin{lstlisting}[language=bash,caption={Connect to AWS from Local Machine}]
ssh -L localhost:8888:localhost:8888 ubuntu@<your instance IP>
source activate conda_tensorflow_p36
jupyter notebook
\end{lstlisting}

\href{https://github.com/awslabs/aws-shell}{The interactive productivity booster for the AWS CLI} provides an useful tool for using AWS. 

\section{Google CoLab}

\href{https://colab.research.google.com}{Google Colaboratory} provides that 12GB GPU support with continuous 12 hours runtime. For RL it requires to render the environment visuals. \href{https://medium.com/@kaleajit27/reinforcement-learning-on-google-colab-9cb2e1ef51e}{Here} is sort of a tutorial to get over that issue \& continue free coding. This is good for play around with free computing resources. However, you only have 12 hours for each session and no storage on the server. You need to install necessary packages every time you start. Use the following in .ipynb and then play around with gym. 

\begin{lstlisting}[language=bash,caption={Google CoLab}] 
# install necessary packages
!pip install gym
!git clone https://github.com/openai/spinningup.git
!pip install -e spinningup  
!pip install tensorflow==1.12.0
!pip install gym pyvirtualdisplay > /dev/null 2>&1
!apt-get install -y xvfb python-opengl ffmpeg > /dev/null 2>&1

# import packages 
from spinup import ppo
import tensorflow as tf
import gym
\end{lstlisting}

\section{Environment Setup}

This environment setup follows the instruction \href{https://spinningup.openai.com/en/latest/user/installation.html#installing-python}{here}. 

\subsection{Local}

Installation of system packages on Mac requires \href{https://brew.sh/}{Homebrew}.% The following \ref{lst:install_spinningup} need only run once at the every beginning. Afterwards, you can start your work after activating your environment -- ``spinningup'' in this example -- by ``source activate spinningup''. 

\begin{lstlisting}[language=bash,caption={Setup SpinningUp Environment}] 
conda create -n spinningup python=3.6

# you need to activate the environment before your start
source activate spinningup   

# install openMPI, need first install Homebrew. 
brew install openmpi  

# installing spinningup
git clone https://github.com/openai/spinningup.git
cd spinningup
pip install -e .

# check install
# try running PPO in the LunarLander-v2 environment with
python -m spinup.run ppo --hid "[32,32]" --env LunarLander-v2 --exp_name installtest --gamma 0.999

# After it finishes training, watch a video of the trained policy with
python -m spinup.run test_policy data/installtest/installtest_s0

# And plot the results with
python -m spinup.run plot data/installtest/installtest_s0

# The last step somehow went wrong with error, will check back later. 

\end{lstlisting}

\subsection{Cloud (AWS)}

Basically the same procedure once you log on to the VM through terminal. The only difference is the operating system is Ubuntu. To install ``OpenMPI'', you will need to use 

\begin{lstlisting}[language=bash,caption={Installing OpenMPI on Ubuntu}] 
sudo apt-get update && sudo apt-get install libopenmpi-dev
\end{lstlisting}

\subsection{OpenAI Gym Intro}

This part is greatly based on the \href{https://gym.openai.com/docs/}{Open AI Gym Tutorial} and \href{https://github.com/openai/gym#environment-specific-installation}{Github Repo}.

\subsubsection{Gym Environment Installation}
To run the code in \href{https://colab.research.google.com}{Google Colab}, you will need to install gym every time you start because your environment is not saved on the serve (no free lunch). Put the following codes at the start of you .ipynb to tell Colab to prepare for the environment. 

\begin{lstlisting}[language=python,caption={Google CoLab Preamble}] 
# Simply install gym using pip
!pip install gym  

# Clone the gym Git repository directly
!git clone https://github.com/openai/gym
!cd gym
!pip install -e .
\end{lstlisting}

Cloning the gym Git repository directly is particularly useful when you’re working on modifying Gym itself or adding environments. You can later run pip install -e .[all] to perform a full installation containing all environments. This requires installing several more involved dependencies, including cmake and a recent pip version.

\textbf{Rendering on a server.} If you're trying to render video on a server, you'll need to connect a fake display. The easiest way to do this is by running under xvfb-run (on Ubuntu, install the xvfb package):

\begin{lstlisting}[language=bash,caption={Installing OpenMPI on Ubuntu}] 
xvfb-run -s "-screen 0 1400x900x24" bash
\end{lstlisting}

\subsubsection{Environment}

After installation, you'll be able to run a few environments right away:
\begin{itemize}
	\item algorithmic
	\item toy\_text
	\item classic\_control (you'll need pyglet to render though)
\end{itemize}

It's better laying with those environments at first, and then later installing the dependencies for the remaining environments. The code for each environment group is housed in its own \href{https://github.com/openai/gym/blob/master/gym/envs}{subdirectory gym/envs}. The specification of each task is in \href{https://github.com/openai/gym/blob/master/gym/envs/__init__.py}{gym/envs/\_\_init\_\_.py}. It's worth browsing through both.

Here’s a bare minimum example of getting something running. This will run an instance of the CartPole-v0 environment for 1000 timesteps, rendering the environment at each step. 


\begin{lstlisting}[language=python,caption={CartPole Env}]  
import gym

#Try replacing ``CartPole-v0'' with ``MountainCar-v0'', ``MsPacman-v0'', or ``Hopper-v1''.
env = gym.make('CartPole-v0') 

env.reset()
for _ in range(1000):
env.render()
env.step(env.action_space.sample()) # take a random action
\end{lstlisting}  \label{lst:cartpole_env}

Some other environments in Gym include ``MountainCar-v0'', ``MsPacman-v0'' and ``Hopper-v1''. Remind that ``MsPacman-v0'' requires the Atari dependency and ``Hopper-v1'' requires the MuJoCo dependencies which necessitate  a \href{https://www.roboti.us/license.html}{MuJoCo license}. Environments all descend from the Env base class.

\textbf{Installing dependencies for specific environments}
If you'd like to install the dependencies for only specific environments, see \href{https://github.com/openai/gym/blob/master/setup.py}{setup.py}. OpenAI maintains the lists of dependencies on a per-environment group basis.

\textbf{Environment groups} include (See this \href{https://colab.research.google.com/drive/1mPXv9Z3rIP3KbUzPzBRXiGtk-j3-IsmU}{Gym\_Environments\_1.ipynb} for details.)
\begin{itemize}
	\item Algorithmic. It contains a variety of algorithmic tasks, such as learning to copy a sequence.
	\item Toy text. Toy environments which are text-based.
	\item Classic control. It comprises of a variety of classic control tasks, which would appear in a typical reinforcement learning textbook.
	\item Atari. The Atari environments are a variety of Atari video games. 
	\item Box2d. It is a 2D physics engine.
	\item MuJoCo. It is a physics engine which can do very detailed efficient simulations with contacts.
	\item Robotics. MuJoCo is a physics engine which can do very detailed efficient simulations with contacts and we use it for all robotics environments. 
\end{itemize}
 
 Run the following code to generate a list of all environments.
 
 \begin{lstlisting}[language=python,caption={Python Code to generate a list of all enironments.}]
 #!/usr/bin/env python
 from gym import envs
 envids = [spec.id for spec in envs.registry.all()]
 for envid in sorted(envids):
 print(envid)
 \end{lstlisting}
 
 Run \href{https://github.com/openai/gym/blob/master/examples/agents/random_agent.py}{examples/agents/random\_agent.py} to run an simple random agent.
 Run \href{https://github.com/openai/gym/blob/master/examples/agents/cem.py}{examples/agents/cem.py} to run an actual learning agent (using the cross-entropy method).

\section{Implementation Plans for Next Week}

\href{https://github.com/dennybritz/reinforcement-learning}{}
\href{https://www.learndatasci.com/tutorials/reinforcement-q-learning-scratch-python-openai-gym/}{}
\href{https://towardsdatascience.com/reinforcement-learning-with-python-8ef0242a2fa2}{}

\subsection{Mar 4th -- Mar 8th.}  

Next week, I am going to delve deeper into the implementation of deep RL. This include the following algorithms.
\begin{itemize}
	\item Deep Q-Network (DQN)
	\item Deep Deterministic Policy Gradients (DDPG)
\end{itemize}

To serve as a guideline, The following algorithms are implemented in the Spinning Up package. 

\begin{itemize}
	\item \href{https://spinningup.openai.com/en/latest/algorithms/vpg.html}{Vanilla Policy Gradient (VPG)}
	\item \href{https://spinningup.openai.com/en/latest/algorithms/trpo.html}{Trust Region Policy Optimization (TRPO)}
	\item \href{https://spinningup.openai.com/en/latest/algorithms/ppo.html}{Proximal Policy Optimization (PPO)}
	\item \href{https://spinningup.openai.com/en/latest/algorithms/ddpg.html}{Deep Deterministic Policy Gradient (DDPG)}
	\item \href{https://spinningup.openai.com/en/latest/algorithms/td3.html}{Twin Delayed} DDPG (TD3)
	\item \href{https://spinningup.openai.com/en/latest/algorithms/sac.html}{Soft Actor-Critic (SAC)}
\end{itemize}


\section{Useful Resources}

\href{https://github.com/openai/curriculum}{OpenAI Curriculum}

\href{https://spinningup.openai.com/en/latest/}{OpenAI Spinning Up in Deep RL}

\href{https://github.com/openai/spinningup}{SpinningUp GitHub Repo}

\href{https://spinningup.openai.com/en/latest/}{OpenAI Spinning Up}




==> exps/99-figure.tex <==
\section{Figures}

\begin{figure}
	\centering
	\begin{subfigure}[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{sample.jpg}
		\caption{Setting 1: $g_{1,1}^\star(x)$}
		%\label{fig:g11true}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{sample.jpg}
		\caption{Setting 2: $g_{1,1}^\star(x)$}
		%\label{fig:g12true}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{sample.jpg}
		\caption{Setting 3: $g_{1,1}^\star(x)$}
		%\label{fig:g13true}
	\end{subfigure}
	
	\begin{subfigure}[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{sample.jpg}
		\caption{Setting 1: $\hat g_{1,1}(x)$}
		%\label{fig:g11hat}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{sample.jpg}
		\caption{Setting 2: $\hat g_{1,2}(x)$}
		%\label{fig:g12hat}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{sample.jpg}
		\caption{Setting 3: $\hat g_{1,3}(x)$}
		%\label{fig:g13hat}
	\end{subfigure}
	\caption{True and estimated $g_{1,1}(x)$ under different settings. Setting 1: $I=100$, $R=3$, $\lambda=5$. Setting 2: $I=400$, $R=3$, $\lambda=5$. Setting 3: $I=400$, $R=3$, $\lambda=10$. Plots for other values of $m\in[3]$ and $r\in[3]$ are similar. }
	\label{fig:g-plots-1}
\end{figure}

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> macros/algorithm.tex <==



% \usepackage{algorithm,algorithmicx,algpseudocode}
% http://shantoroy.com/latex/how-to-write-algorithm-in-latex/
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
%\usepackage{algorithm}
%\usepackage{algpseudocode}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}} % require \usepackage{xcolor}
\SetCommentSty{mycommfont}

\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\SetKwInput{KwInitialize}{Initialize}    % set initialization

==> macros/box-theorems.tex <==
% more info here
% https://texblog.org/2015/09/30/fancy-boxes-for-theorem-lemma-and-proof-with-mdframed/

\usepackage[framemethod=TikZ]{mdframed} % box environment & flexible box designs

% or
\usepackage{fancybox}

==> macros/code.tex <==

%%
%%  code listing macros
%%

%% refs: https://www.overleaf.com/learn/latex/Code_listing

\usepackage{listings}             % Include the listings-package
\lstset{basicstyle=\ttfamily,
	showstringspaces=false,
	commentstyle=\color{red},
	keywordstyle=\color{blue}
}

==> proofs/1-NP_hard.tex <==

\subsection{Proof of Theorem \ref{thm:NP-hard_exact}}
\label{ssec:proof_NPhard_exact}
\proof{Proof.}

% We prove that the $p$-Hypercube problem is NP-hard by a polynomial reduction of the $p$-Median problem, which is known to be NP-hard \citep{kariv1979algorithmic}. 

% In the $p$-Hypercube problem, recall that $\lambda_j$ is the call arrival rate from subregion $j$, $P(\boldsymbol{b})$ is the probability of being in state $\boldsymbol{b}$, and $\Pi_j$ is the probability that all units that can serve sub-region $j$ are busy. We define the weight of subregion $j$, $w_j$, as the normalized arrival rate $\lambda_j/\sum_{k\in J} \lambda_k$, and $q_{i j}(\boldsymbol{x})$ is the fraction of calls in subregion $j$ that are responded to by the unit at location $i$ given unit configuration $\boldsymbol{x}$, as given by
% \begin{equation}
% q_{i j}(\boldsymbol{x})=  \frac{\sum_{\boldsymbol{b} \in S_{ij}(\boldsymbol{x})} \lambda_j P(\boldsymbol{b})}{\sum_{k\in J} \lambda_k \left(1-\Pi_j\right)} = w_j  \frac{\sum_{\boldsymbol{b} \in S_{ij}(\boldsymbol{x})} P(\boldsymbol{b})}{1-\Pi_j}.
% \end{equation}

% Given an instance $\mathcal{I}$ of the $p$-Median problem, we construct an instance $\mathcal{I}^\prime$ of the $p$-Hypercube problem by setting $S_{ij}(\boldsymbol{x})$ in $\mathcal{I}^\prime$ such that 
% \begin{equation}
% \frac{\sum_{\boldsymbol{b} \in S_{ij}(\boldsymbol{x})} P(\boldsymbol{b})}{1-\Pi_j} = y_{ij}. \label{eq:NP_satisfy}
% \end{equation}

% In $\mathcal{I}^\prime$, the set $S_{ij}(\boldsymbol{x})$ denotes states where the unit at location $i$ is designated for calls from subregion $j$. We observe that a significant challenge is the binary assignment requirement of the $p$-Median, which dictates that each sub-region $j$ be assigned exclusively to one location $i$. Conversely, the $p$-Hypercube model does not inherently impose such constraints. To address this, we establish the assignment rule for the $p$-Hypercube problem as follows: if $y_{ij}=1$ in $\mathcal{I}$, then in $\mathcal{I}^\prime$, assign unit $i$ as the primary responder and the sole unit to cover sub-region $j$. Should unit $i$ be occupied, any incoming calls from sub-region $j$ are disregarded. Furthermore, we assign $S_{ij}(\boldsymbol{x}) = \varnothing$ for all $i$ and $j$ pairs in $\mathcal{I}^\prime$ where $y_{ij}=0$ in $\mathcal{I}$.

% Consequently, for $y_{ij}=0$ in $\mathcal{I}$, $\sum_{\boldsymbol{b} \in S_{ij}(\boldsymbol{x})} P(\boldsymbol{b}) = 0$ in $\mathcal{I}^\prime$. Additionally, for $y_{ij}=1$ in $\mathcal{I}$, we derive
% \begin{equation}
%     \frac{\sum_{\boldsymbol{b} \in S_{ij}(\boldsymbol{x})} P(\boldsymbol{b})}{1-\Pi_j} = \frac{1-\rho_i}{1-\Pi_j}=1. 
% \end{equation}
% The first equality arises because, when each sub-region $j$ is assigned exclusively to one location $i$, then $S_{ij}(\boldsymbol{x})$ represents the set of states where the unit at location $i$ is available. Therefore, summing over the probabilities of all such states, $\sum_{\boldsymbol{b} \in S_{ij}(\boldsymbol{x})} P(\boldsymbol{b})$, equates to the probability that the unit at location $i$ is available, which is $1-\rho_i$, with $\rho_i$ representing the unit's utilization. The second equality is valid because the fraction of calls from sub-region $j$ that are blocked, $\Pi_j$, equals the probability that the unit at location $i$ is busy, $\rho_i$, when the unit from location $i$ exclusively serves sub-region $j$.

% Consequently, \eqref{eq:NP_satisfy} holds, and all constraints in the $p$-Median problem are met through such an equivalence relationship. By this construction, we ensure that a solution to $\mathcal{I}$ corresponds to a solution to $\mathcal{I}^\prime$ and vice versa. Consequently, if we solve $\mathcal{I}^\prime$ optimally, we obtain an optimal solution to $\mathcal{I}$ as well, thus proving the reduction from the $p$-Median problem to the $p$-Hypercube problem in polynomial time. Since the $p$-Median problem is already known to be NP-hard, we conclude that the $p$-Hypercube problem is also NP-hard.

\Halmos

\endproof




==> proofs/2-lower_bound.tex <==


\subsection{Proof of Theorem \ref{thm_low_bound_exact}}
\label{ssec_lower_bound_proof_exact}
\proof{Proof.}

We prove this theorem by first showing that the feasible region of $p$-Hypercube is a subset of the feasible region of the $p$-Median problem, and the optimal value of the $p$-Median problem (denoted by $\text{OPT}_M$) is a lower bound to the optimal value of the $p$-Hypercube problem (denoted by $\text{OPT}_H$). Let $\tilde{y}_{ij} = \sum_{\boldsymbol{b} \in S_{ij}(\boldsymbol{x})} P(\boldsymbol{b})/(1-\Pi)$, where $\Pi$ is the probability that all units are busy, also known as the blocking probability.
We first show that $\sum_{i\in I} \tilde{y}_{ij} = 1$ for all $j\in J$.

Recall that $S_{ij}(\boldsymbol{x})$ is the set of states in which the unit at location $i$ is assigned to calls from subregion $j$ given the set of unit locations $\boldsymbol{x}$. Thus, $\boldsymbol{b} \in S_{ij}(\boldsymbol{x})$ indicates that in state $\boldsymbol{b}$, unit $i$ is the first preferred available unit. Let $\boldsymbol{B}$ denote the set of all possible states given the set of unit locations $\boldsymbol{x}$. The cardinality of $\boldsymbol{B}$ is $|\boldsymbol{B}| = 2^{p}$.  We have 
{
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
\begin{align*}
    \tilde{y}_{ij} &= \frac{\sum_{\boldsymbol{b} \in S_{ij}(\boldsymbol{x})} P(\boldsymbol{b}) }{1-\Pi}= \frac{\sum_{\boldsymbol{b} \in \boldsymbol{B}} P(\boldsymbol{b}) \mathbbm{1}_{\{\boldsymbol{b} \in S_{ij}(\boldsymbol{x})\}} }{1-\Pi}= \frac{\sum_{\boldsymbol{b} \in \boldsymbol{B}} P(\boldsymbol{b}) \mathbbm{1}_{\{b_i = 0\}} \prod_{k<\eta_{j}(i)} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}} }{1-\Pi},
\end{align*}
}
where $\gamma_{jl}$ is the index of the $l$-th preferred unit in subregion $j$ in the preference list, and $\eta_{j}(i)$ is the preference rank of unit $i$ in subregion $j$. In the last line of the above equation, $\prod_{k<\eta_{j}(i)} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}} $ indicates whether all units with  preference ranks higher than unit $i$ are busy in state $\boldsymbol{b}$.. 

Let $X_{ij}^{\boldsymbol{b}} = \sum_{i\in I} \mathbbm{1}_{\{b_i = 0\}} \prod_{k<\eta_{j}(i)} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}}$. We have
{
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
\begin{align*}
    \sum_{i\in I} \tilde{y}_{ij} &= \sum_{i\in I} \frac{\sum_{\boldsymbol{b} \in \boldsymbol{B}} P(\boldsymbol{b}) \mathbbm{1}_{\{b_i = 0\}} \prod_{k<\eta_{j}(i)} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}} }{1-\Pi}\\
&= \frac{\sum_{\boldsymbol{b} \in \boldsymbol{B}} P(\boldsymbol{b})\sum_{i\in I} \mathbbm{1}_{\{b_i = 0\}} \prod_{k<\eta_{j}(i)} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}} }{1-\Pi}=\frac{\sum_{\boldsymbol{b} \in \boldsymbol{B}} P(\boldsymbol{b}) X_{ij}^{\boldsymbol{b}}}{1-\Pi}.
\end{align*}
}
Denote $\boldsymbol{b}^*$ as the state where all units are busy. We first claim that $X_{ij}^{\boldsymbol{b}^*} = 0$, which follows directly from the fact that $b_i = 1$ for all $i$ in state $\boldsymbol{b}^*$, and $\mathbbm{1}_{\{b_i = 0\}} = 0$ for all $i$.

We next show that $X_{ij}^{\boldsymbol{b}} = 1$ for all $\boldsymbol{b} \in \boldsymbol{B} \setminus \boldsymbol{b}^*$. Denote by $\mathscr{G}_{j}^l$ the set of states in which the $l-1$ most preferred units are busy and the $l$-th preferred unit is available in subregion $j$. We have 
{\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
\begin{equation}
    \mathscr{G}_{j}^l = \{\boldsymbol{b}: b_{\gamma_{jl}}=0, b_{\gamma_{jk}}=1, \ \forall k < l, \boldsymbol{b}\in \boldsymbol{B}\}.
\end{equation}
We claim that
\begin{equation}
    \cup_{l=1}^N  \mathscr{G}_{j}^l \cup \{\boldsymbol{b}^*\}=\boldsymbol{B}, \qquad \forall j\in J,
\end{equation}
}
since all states except for $\boldsymbol{b}^*$ belong to $\cup_{l=1}^N  \mathscr{G}_{j}^l$ by construction of the set $\mathscr{G}_{j}^l$. 

For all states in which the most preferred unit is available, i.e., $\forall \boldsymbol{b}\in \mathscr{G}_{j}^1$, we have
{
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
\begin{align*}
    X_{ij}^{\boldsymbol{b}} &= \mathbbm{1}_{\{b_{\gamma_{j1}} = 0\}} + \sum_{i \not= \gamma_{j1}} \mathbbm{1}_{\{b_i = 0\}} \prod_{k<\eta_{j}(i)} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}} = 1 + \sum_{i \not= \gamma_{j1}} \mathbbm{1}_{\{b_i = 0\}} \mathbbm{1}_{\{b_{\gamma_{j1}} = 1\}} \prod_{1<k<\eta_{j}(i)} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}} = 1,
\end{align*}
}
since $\forall \boldsymbol{b}\in \mathscr{G}_{j}^1$ we have $\mathbbm{1}_{\{b_{\gamma_{j1}} = 0\}}=1$ and $\mathbbm{1}_{\{b_{\gamma_{j1}} = 1\}}=0$ because $\gamma_{j1}$ is the most preferred free unit in subregion $j$. 

For all states in which the $l-1$ most preferred units are busy and the $l$-th preferred unit is available, i.e., $\forall \boldsymbol{b}\in \mathscr{G}_{j}^l$ and $j>1$, we have
{
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
\begin{align*}
    X_{ij}^{\boldsymbol{b}} &= \sum_{i: \eta_{j}(i)<l} \mathbbm{1}_{\{b_i = 0\}} \prod_{k<\eta_{j}(i)} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}} + \mathbbm{1}_{\{b_{\gamma_{jl}} = 0\}} \prod_{k<l} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}}+ \sum_{i: \eta_{j}(i)>l} \mathbbm{1}_{\{b_i = 0\}} \prod_{k<\eta_{j}(i)} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}}\\
&= 1 + \sum_{i: \eta_{j}(i)>l} \mathbbm{1}_{\{b_i = 0\}} \bigg(\prod_{k<l} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}}\bigg) \mathbbm{1}_{\{b_{\gamma_{jl}}= 1\}} \bigg(\prod_{l<k<\eta_{j}(i)} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}}\bigg) = 1,
\end{align*}
}
since $\forall \boldsymbol{b}\in \mathscr{G}_{j}^l$ we have $\mathbbm{1}_{\{b_{\gamma_{jl}} = 0\}}=1$ and $\mathbbm{1}_{\{b_{\gamma_{jl}} = 1\}}=0$ by definition, and $\mathbbm{1}_{\{b_i = 0\}}=0$ for $\eta_{j}(i)<l$ and $\prod_{k<l} \mathbbm{1}_{\{b_{\gamma_{jk}} = 1\}}=1$.

Combining the above equations, we have 
{
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
\begin{align*}
    \sum_{i\in I} \tilde{y}_{ij} &= \frac{\sum_{\boldsymbol{b}\in \boldsymbol{B}} P(\boldsymbol{b}) X_{ij}^{\boldsymbol{b}}}{1-\Pi}= \frac{\sum_{\boldsymbol{b}\in \boldsymbol{B} \setminus \boldsymbol{b}^*} P(\boldsymbol{b}) X_{ij}^{\boldsymbol{b}} + \Pi\cdot X_{ij}^{\boldsymbol{b}^*} }{1-\Pi}=\frac{1-\Pi}{1-\Pi} \label{eq_sum}= 1.
\end{align*}
}
We obtain \eqref{eq_sum} because $X_{ij}^{\boldsymbol{b}}=1$ for $\boldsymbol{b}\in \boldsymbol{B} \setminus \boldsymbol{b}^*$, $X_{ij}^{\boldsymbol{b}^*} = 0$, and $\sum_{\boldsymbol{b}\in B } P(\boldsymbol{b})=1$. 

Thus, we have demonstrated that $\sum_{i \in I} \tilde{y}_{ij} = 1$ for all $j \in J$, fulfilling Constraint \eqref{eq:y_sum} of the $p$-Median problem, while the $p$-Hypercube problem inherently satisfies Constraint \eqref{eq:x_sum}. We further argue that Constraint \eqref{eq:y_valid} is met. This is because, for $x_{i}=0$, indicating no unit at location $i$, $S_{ij}=\emptyset$ leads to $\tilde{y}_{ij} = 0$. For $x_{i}=1$, given that $\sum_{i \in I} \tilde{y}_{ij} = 1$ and each $\tilde{y}_{ij}$ is non-negative by definition, Constraint \eqref{eq:y_valid} is met. Additionally, by defining $w_j = \lambda_j/\sum_{k \in J} \lambda_k$, we align the objective function of the $p$-Hypercube problem with that of the $p$-Median.

With this transformation and any specified dispatch policy, the $p$-Hypercube simplifies to the following:
{
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
\begin{align}
\text{OPT}_{H} = \min_{\boldsymbol{x}, \boldsymbol{y}} & \sum_{i \in I} \sum_{j \in J} w_j (\tau_i + t_{i j}) \tilde{y}_{i j} \\
\text { s.t. } 
&\sum_{i \in I} x_{i}=p,\\
& \sum_{i \in I} \tilde{y}_{i j}=1, \forall j \in J, \\
& \tilde{y}_{i j} \leq x_{i}, \forall i \in I, \forall j \in J,\\
& x_{i} \in\{0,1\}, \forall i \in I
\end{align}
}
where $\tilde{y}_{i j} =\sum_{\boldsymbol{b} \in S_{ij}(\boldsymbol{x})} P(\boldsymbol{b})/(1-\Pi) \in [0,1]$ is fixed and determined by the solution $\boldsymbol{x} = \{x_1, \cdots, x_N\}$ and the assignment rule. 

Next, we show that $\text{OPT}_H \geq \text{OPT}_M$ always holds. To prove this, we argue that for any feasible solution $\boldsymbol{x} = {x_1, \ldots, x_N}$ (including the optimal solution for the $p$-Hypercube problem), we have
\begin{equation}
    \sum_{i \in I} w_j (\tau_i + t_{i j}) y^*_{i j}\leq \sum_{i \in I} w_j (\tau_i + t_{i j}) \tilde{y}_{i j},
\end{equation}
where $y^*_{i j}$ is the optimal solution to the $p$-Median problem given $\boldsymbol{x}$. The basic idea is to show that for each sub-region $j\in J$, we have
\begin{equation}
    \sum_{i \in I} w_j (\tau_i + t_{i j}) y^*_{i j} = \min_{i: x_{i}=1} w_j (\tau_i + t_{i j}), \label{eq:_obj_left}
\end{equation}
and 
\begin{equation}
    \sum_{i \in I} w_j (\tau_i + t_{i j}) \tilde{y}_{i j} \geq \min_{i: x_{i}=1} w_j (\tau_i + t_{i j}). \label{eq:_obj_right}
\end{equation}

To see \eqref{eq:_obj_left} holds, we note that we set no constraint on $y_{i j}$ across sub-regions $j$ when $x_i=1$. Thus, for each sub-region $j\in J$, the optimal value is attained at the minimum value of $w_j (\tau_i + t_{i j})$. For \eqref{eq:_obj_right}, we have
\begin{equation}
    \sum_{i \in I} w_j (\tau_i + t_{i j}) \tilde{y}_{i j}  \geq \sum_{i \in I} \tilde{y}_{i j} \big(\min_{i: x_{i}=1} w_j (\tau_i + t_{i j}) \big)= \min_{i: x_{i}=1} w_j (\tau_i + t_{i j}).
\end{equation}

Thus, we conclude that for any feasible solution $\boldsymbol{x} = \{x_1, \cdots, x_N\}$ of $p$-Hypercube, the optimal value for the $p$-Median problem is no larger than that for the $p$-Hypercube problem. 
Therefore, the optimal value of the $p$-Median problem is a lower bound on the optimal value of the $p$-Hypercube problem, i.e.,
\begin{equation}
\text{OPT}_H \geq \text{OPT}_M.
\end{equation}
\Halmos
\endproof
% Next, we show that the gap between the two values approaches 0 as the minimum service rate $\mu = \min_i \mu_i$ approaches infinity, i.e., 
% \begin{equation}
%     \lim_{\mu\rightarrow \infty}\text{OPT}_H - \text{OPT}_M = 0.
% \end{equation}



